BANGS: Game-Theoretic Node Selection for Graph Self-Training

Graph self-training is a semi-supervised learning method that iteratively selects a set of unlabeled data to retrain the underlying graph neural network (GNN) model and improve its prediction performance. While selecting highly confident nodes has proven effective for self-training, this pseudo-labeling strategy ignores the combinatorial dependencies between nodes and suffers from a local view of the distribution. To overcome these issues, we propose BANGS, a novel framework that unifies the labeling strategy with conditional mutual information as the objective of node selection. Our approach -- grounded in game theory -- selects nodes in a combinatorial fashion and provides theoretical guarantees for robustness under noisy objective. More specifically, unlike traditional methods that rank and select nodes independently, BANGS considers nodes as a collective set in the self-training process. Our method demonstrates superior performance and robustness across various datasets, base models, and hyperparameter settings, outperforming existing techniques. The codebase is available on https://github.com/fangxin-wang/BANGS .

==> related_work.tex <==
\label{sec. review}

% \fx{Should I add some general self-training works?} \sm{No need. Also, we need to merge this in the introduction may be: kind of thinking like this structure \url{https://proceedings.neurips.cc/paper_files/paper/2022/file/8d492b8a6201d83d1015af9e264f0bf2-Paper-Conference.pdf}}

For full usage of unsupervised information, early work in graph self-training~\cite{li2018deeper} proposes to boost GCN models by the expanded label set. This method is extended to 
\textbf{M3S}, a multiple stage self-training strategy by~\cite{sun2020multi}, where deep-clustering outputs are first aligned to labeled data, and then used to assign pseudo-labels for each unlabeled data point in the embedding space. 
Designed for graph self-training with very few labels, \cite{zhou2023effective} develop a stabilized pseudo-labeling technique using class imbalance and negative sampling regularization technique. \cite{botao2023deep} prove with under graph perturbation invariant property, a lower bound of self-training prediction accuracy is correlated with GNN prediction consistency and confidence. Consequently, they propose \textbf{CPL}, which select nodes with high average confidence and consistent predicted labels by multi-view augmented predictors.


%by measuring how much one node can represent its surrounding neighborhood and discriminate an arbitrary neighborhood.
%Based on the conjecture that a high softmax score can provide a low-accurate estimation when the first and second top prediction scores are similar, \cite{pedronette2021rank} proposes margin confidence that globally ranks the nodes to be selected. 
%Aware of graph structure information, \cite{yang2021self} propose a topology update to remove inter-class edges and add intra-class edges, and then apply the self-training mechanism.

%\cite{li2023informative} considers an unlabeled node to be informative when it can maximally reflect its local neighborhood. By integrating this informativeness measure with model prediction probabilities, they select pseudo-label nodes with maximum information gains to reduce redundancy. 


%Graph self-training performance are also believed to improved by well-calibrated GNNs and often employed as one of the downstream tasks for GNN confidence calibration \cite{wang2021confident,hsu2022makes}. Though sole calibration have been shown to improve GNN self-training performance, few work examine whether calibration can further enhance performance when combined with other strategies.

%In a closer relation to the focus of this work, some previous works intend to estimate uncertainty with consideration for graph structure at the node selection stage. \cite{zhao2021entropy} proposes to add an entropy-aggregation layer to GCN for confidence estimation, along with a disentangled checking part based on information aggregation and SVM for pseudo-label assignment. \cite{ghayekhloo2023clp} propagate the confidence scores of the labels along with the pseudo-labels assigned to the nodes, where the confidence of an unlabeled node is computed by the feature and embedding similarity between all labeled nodes. 


% Elements of Self-training: 1) uncertainty estimation 2) label selection 3) label assignment 
%In general self-training settings, multiple labeling strategies have been developed, especially in pseudo-label selection. Many works ~\cite{tur2005combining,cascante2021curriculum,zhang2021flexmatch} focus on optimizing confidence thresholds to adapt for distribution shift in each iteration. As an example, Curriculum Pseudo Labeling (CPL) utilizes a curriculum learning approach to adaptively adjust confidence thresholds of unlabeled data according to the model’s learning status in different classes~\cite{zhang2021flexmatch}. The main idea of this work is the increasing number of pseudo-labeled examples raises the inducing error~\cite{feofanov2019transductive}, in which case the confidence threshold needs reduction. 

%Besides the distribution shift, another intrinsic problem of self-training is the inevitably noisy pseudo-labels. Therefore, another bunch of works focuses on denoising self-training, e.g., co-training with two classifiers crossingly~\cite{chen2022debiased}, regularization~\cite{miyato2018virtual,zou2019confidence}, and mislabeled transition matrix~\cite{patrini2017making,liu2022confidence}. Yet due to the special information aggregation mechanism, information redundancy seems to be a more evident problem when applying self-training for GNN. To address this, \cite{liu2022confidence,li2023informative} select nodes with high information gain instead of high confidence. Entropy is commonly used to estimate the information gained from labeling in those papers, which, however, is not always helpful to all graph learning tasks according to \cite{zhao2020uncertainty}.

